Taichi: An Open-Source Computer Graphics Library

An ideal software system in computer graphics should be a combination of innovative ideas, solid software engineering and rapid development. However, in reality these requirements are seldom met simultaneously. In this paper, we present early results on an open-source library named Taichi (http://taichi.graphics), which alleviates this practical issue by providing an accessible, portable, extensible, and high-performance infrastructure that is reusable and tailored for computer graphics. As a case study, we share our experience in building a novel physical simulation system using Taichi.

==> Commands.tex <==
% vectors, matrices, sets, and functions
\renewcommand{\vec}[1]{\boldsymbol{\mathrm{#1}}}
\newcommand{\mat}[1]{\boldsymbol{\mathrm{#1}}}
\let\set=\mathcal
\let\func=\mathrm

% common symbols
\newcommand{\N}{\mbox{\rm \hbox{I\kern-.15em\hbox{N}}}}
\newcommand{\R}{\mbox{\rm \hbox{I\kern-.15em\hbox{R}}}}
\newcommand{\laplace}{\Delta}
\newcommand{\grad}{\nabla}
\newcommand{\strain}{\vec{\epsilon}}
\newcommand{\stress}{\vec{\sigma}}

\newcommand{\minipar}[1]{\vspace{.75ex}\noindent\textbf{#1}\hspace{2ex}}

%\renewcommand{\SS}{{\mathcal{E}}}
\newcommand{\RS}{{\mathcal{F}}}
\newcommand{\ES}{{\mathcal{E}}}

% some math commands
\def \N {\mbox{\rm \hbox{I\kern-.15em\hbox{N}}}}
\def \R {\mbox{\rm \hbox{I\kern-.15em\hbox{R}}}}
\def \laplace {\Delta}
\def \grad {\nabla}
\def \dprod {\mspace{-1mu} \cdot \mspace{-1mu}}
\def \tprod {\mspace{-1mu} : \mspace{-1mu}}
\newcommand{\of}[1]{\mspace{-3mu}\left( #1 \right)}
\newcommand{\ofx}{\of{\vec{x}}}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\norm}[1]{\left\Vert {#1} \right\Vert}
\newcommand{\D}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\twovec}[2]{\left[\begin{array}{c}#1\\#2\end{array}\right]}
\newcommand{\threevec}[3]{\left[\begin{array}{c}#1\\#2\\#3\end{array}\right]}
\renewcommand{\matrix}[2]{\left[\begin{array}{#1}#2\end{array}\right]}
\newcommand{\dV}{\,\mathrm{d}\Omega}
\newcommand{\dA}{\,\mathrm{d}\set{S}}
\newcommand{\ds}{\,\mathrm{d}\Gamma}

% references and abbreviations
\newcommand{\refsec}[1]{Section~\ref{sec:#1}}
\newcommand{\Eq}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\Fig}[1]{Fig.~\ref{fig:#1}}
\newcommand{\Figure}[1]{Figure~\ref{fig:#1}}
\newcommand{\Table}[1]{Table~\ref{tab:#1}}
\newcommand{\eq}[1]{(\ref{eq:#1})}

%specific commands from the hfem paper
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bm}{\mathbf{m}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bl}{\mathbf{l}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\bw}{\vec{w}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bj}{\mathbf{j}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bXi}{\boldsymbol{\Xi}}

\newcommand{\fint}{\mathbf{f}_\mathrm{int}}
\newcommand{\fext}{\mathbf{f}_\mathrm{ext}}

\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\btheta}{\boldsymbol{\theta}}

\newcommand{\comment}[3]
{
%\textcolor{#3}{#1: #2}
}

\newcommand{\MS}[1]
{
\comment{MS}{#1}{red}
}

\newcommand{\changed}[1]
{
%\textcolor{red}{#1}
#1
}


